Deeply Learning Deep Inelastic Scattering Kinematics

We study the use of deep learning techniques to reconstruct the kinematics of the neutral current deep inelastic scattering (DIS) process in electron-proton collisions. In particular, we use simulated data from the ZEUS experiment at the HERA accelerator facility, and train deep neural networks to reconstruct the kinematic variables $Q^2$ and $x$. Our approach is based on the information used in the classical construction methods, the measurements of the scattered lepton, and the hadronic final state in the detector, but is enhanced through correlations and patterns revealed with the simulated data sets. We show that, with the appropriate selection of a training set, the neural networks sufficiently surpass all classical reconstruction methods on most of the kinematic range considered. Rapid access to large samples of simulated data and the ability of neural networks to effectively extract information from large data sets, both suggest that deep learning techniques to reconstruct DIS kinematics can serve as a rigorous method to combine and outperform the classical reconstruction methods.

==> Makefile <==
#ulimit -u 10000
latexfile=DISML
newname?=DISML
STYLE=epjc

LUALATEX=  export LANG="en_US.UTF-8";  lualatex
LATEX=  export LANG="en_US.UTF-8";  pdflatex -halt-on-error -shell-escape -enable-write18
BIBTEX=bibtex


ifeq ($(STYLE),draft)
	STYLE_SPECIFIC_FILES=zeus_paper.cls $(latexfile)-draft.tex lineno.sty mcite.sty units.sty
endif

ifeq ($(STYLE),arxiv)
	STYLE_SPECIFIC_FILES=zeus_paper.cls $(latexfile)-arxiv.tex mcite.sty units.sty 
endif

ifeq ($(STYLE),epjc)
	STYLE_SPECIFIC_FILES=svjour.cls  svepj.clo $(latexfile)-epjc.tex   
endif

ifeq ($(STYLE),jhep)
	STYLE_SPECIFIC_FILES=jheppub.sty $(latexfile)-jhep.tex JHEP.bst
endif


all: $(latexfile)-$(STYLE).pdf


tables=Tables/centralresolutionsimple Tables/centralresolutionsimpleepjc Tables/table2cdmcentral.dat  Tables/tablecdmcentral.dat


figures=Figures/MSE-figure0.pdf \
        Figures/Q2resolution1-figure0.pdf \
        Figures/Q2resolution2-figure0.pdf \
        Figures/Q2resolution3-figure0.pdf \
        Figures/Q2resolution4-figure0.pdf \
        Figures/Q2resolution5-figure0.pdf \
        Figures/Q2resolution6-figure0.pdf \
        Figures/Q2resolution7-figure0.pdf \
        Figures/Q2resolution8-figure0.pdf \
        Figures/xresolution1-figure0.pdf \
        Figures/xresolution2-figure0.pdf \
        Figures/xresolution3-figure0.pdf \
        Figures/xresolution4-figure0.pdf \
        Figures/xresolution5-figure0.pdf \
        Figures/xresolution6-figure0.pdf \
        Figures/xresolution7-figure0.pdf \
        Figures/xresolution8-figure0.pdf \
        Figures/DIS0-figure0.pdf   \
        Figures/DIS1a-figure0.pdf  \
        Figures/DIS2a-figure0.pdf  \
        Figures/DIS3a-figure0.pdf  \
        Figures/DIS4a-figure0.pdf  \
        Figures/DIS5a-figure0.pdf  \
        Figures/DIS6a-figure0.pdf  \
        Figures/DIS7a-figure0.pdf  \
        Figures/DIS8a-figure0.pdf  \
        Figures/DIS9a-figure0.pdf  \
        Figures/DIS10a-figure0.pdf  \
        Figures/DIS11a-figure0.pdf  \
        Figures/Q22dresolution1-figure0.pdf \
        Figures/Q22dresolution2-figure0.pdf \
        Figures/Q22dresolution3-figure0.pdf \
        Figures/Q22dresolution4-figure0.pdf \
        Figures/Q22dresolution5-figure0.pdf \
        Figures/Q22dresolution6-figure0.pdf \
        Figures/Q22dresolution7-figure0.pdf \
        Figures/Q22dresolution8-figure0.pdf \
        Figures/x2dresolution1-figure0.pdf \
        Figures/x2dresolution2-figure0.pdf \
        Figures/x2dresolution3-figure0.pdf \
        Figures/x2dresolution4-figure0.pdf \
        Figures/x2dresolution5-figure0.pdf \
        Figures/x2dresolution6-figure0.pdf \
        Figures/x2dresolution7-figure0.pdf \
        Figures/x2dresolution8-figure0.pdf \
        Figures/Q2x-figure0.pdf





tar:  Makefile figurelist-$(STYLE).txt $(constanttables) $(tables)  $(latexfile)-def.tex  \
	$(latexfile).bib $(latexfile)-abs.tex $(latexfile)-txt.tex $(latexfile)-tab.tex $(latexfile)-fig.tex  $(STYLE_SPECIFIC_FILES)
	rm -rf TAR
	mkdir -p TAR
	mkdir -p TAR/Figures
	mkdir -p TAR/Tables
	cp Makefile   $(latexfile).bst $(latexfile).bib   $(latexfile)-def.tex $(latexfile)-abs.tex $(latexfile)-txt.tex $(latexfile)-tab.tex $(latexfile)-fig.tex    $(STYLE_SPECIFIC_FILES) TAR
	cp $(tables) TAR/Tables
	cp $(figures) TAR/Figures
	for a in $$(cat   figurelist-$(STYLE).txt); do\
		cp $$a TAR/Figures;\
	done	
	sed -i 's@'$(latexfile)'@'$(newname)'@g' TAR/*tex	
	sed -i 's@'$(latexfile)'@'$(newname)'@g' TAR/Makefile
	sed -i 's@^STYLE.*@STYLE='$(STYLE)'@g' TAR/Makefile
	sed -i '/@artic/achecked={2},'     TAR/*bib	
	sed -i '/@inproceed/achecked={2},' TAR/*bib	
	sed -i '/@phdthesis/achecked={2},' TAR/*bib	

ifeq ($(STYLE),epjc)
	sed -i 's@\[htbp\]@@g' TAR/$(latexfile)-tab.tex
	sed -i 's@c|@c@g' TAR/$(latexfile)-tab.tex
	sed -i 's@|c@c@g' TAR/$(latexfile)-tab.tex
	sed -i 's@{|c}@c@g' TAR/$(latexfile)-tab.tex
	sed -i 's@{c|}@c@g' TAR/$(latexfile)-tab.tex
	sed -i 's@}|@}@g' TAR/$(latexfile)-tab.tex
endif
	mv TAR/$(latexfile).bst TAR/$(newname).bst 
	mv TAR/$(latexfile).bib TAR/$(newname).bib 
ifeq ($(STYLE),jhep)
	rm TAR/$(newname).bst 
endif
	mv TAR/$(latexfile)-$(STYLE).tex TAR/$(newname)-$(STYLE).tex
	mv TAR/$(latexfile)-txt.tex TAR/$(newname)-txt.tex
	mv TAR/$(latexfile)-abs.tex TAR/$(newname)-abs.tex
	mv TAR/$(latexfile)-tab.tex TAR/$(newname)-tab.tex
	mv TAR/$(latexfile)-def.tex TAR/$(newname)-def.tex
	mv TAR/$(latexfile)-fig.tex TAR/$(newname)-fig.tex
ifeq ($(STYLE),arxiv)
	#####-->A trick to get the bib file for axiv build system
	$(MAKE) -C TAR
	mv TAR/$(newname)-$(STYLE).bbl  TAR/$(newname)-$(STYLE).bbl.temp
	$(MAKE) -C TAR clean
	mv TAR/$(newname)-$(STYLE).bbl.temp  TAR/$(newname)-$(STYLE).bbl
endif
ifeq ($(STYLE),epjc)
	#####-->A trick to get the bib file for axiv build system
	$(MAKE) -C TAR
	mv TAR/$(newname)-$(STYLE).bbl  TAR/$(newname)-$(STYLE).bbl.temp
	$(MAKE) -C TAR clean
	mv TAR/$(newname)-$(STYLE).bbl.temp  TAR/$(newname)-$(STYLE).bbl
endif
ifeq ($(STYLE),jhep)
	#####-->A trick to get the bib file for axiv build system
	$(MAKE) -C TAR
	mv TAR/$(newname)-$(STYLE).bbl  TAR/$(newname)-$(STYLE).bbl.temp
	$(MAKE) -C TAR clean
	cp TAR/$(newname)-$(STYLE).bbl.temp  TAR/$(newname).bbl
	mv TAR/$(newname)-$(STYLE).bbl.temp  TAR/$(newname)-$(STYLE).bbl
endif

	tar -zcvf   $(newname).tar.gz -C TAR . 
	rm -rf $(newname).zip; cd TAR; zip ../$(newname).zip ./*/* ./*; cd ..


       


$(latexfile)-$(STYLE).fls: $(constanttables) $(tables) \
                    $(latexfile).bib $(latexfile)-abs.tex $(latexfile)-txt.tex $(latexfile)-tab.tex\
                     $(latexfile)-fig.tex   $(STYLE_SPECIFIC_FILES)
		pdflatex -recorder $(latexfile)-$(STYLE).tex
figurelist-$(STYLE).txt:  $(latexfile)-$(STYLE).fls
		cat $(latexfile)-$(STYLE).fls | grep pdf | grep Figures | sed 's@\./@@g' |sort | cut -f2 -d' '| uniq  > figurelist-$(STYLE).txt
constanttables=


$(latexfile)-$(STYLE).pdf :  $(figures) $(constanttables) $(tables) \
                    $(latexfile).bib $(latexfile)-abs.tex $(latexfile)-txt.tex $(latexfile)-tab.tex\
                     $(latexfile)-fig.tex  $(STYLE_SPECIFIC_FILES)
	
	$(LATEX) $(latexfile)-$(STYLE)
	$(LATEX) $(latexfile)-$(STYLE)
	$(BIBTEX) $(latexfile)-$(STYLE)
	$(BIBTEX) $(latexfile)-$(STYLE)
ifeq ($(STYLE),epjc)
	sed -i 's@\\mbox{}.*@@g'  $(latexfile)-$(STYLE).bbl
endif
ifeq ($(STYLE),arxiv)
	sed -i 's@\\mbox{}.*@@g'  $(latexfile)-$(STYLE).bbl
endif
	$(LATEX) $(latexfile)-$(STYLE)
	$(LATEX) $(latexfile)-$(STYLE)


pdf : $(latexfile)-$(STYLE).pdf

$(latexfile).rws: $(latexfile)-dict.txt
	aspell --lang=en create master ./$(latexfile).rws < ./$(latexfile)-dict.txt

spell: $(latexfile).rws
		for a in $$(ls -1 $(latexfile)-*.tex); do\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		echo $$a;\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		aspell  --add-extra-dicts=./$(latexfile).rws  -t \
			--add-tex-command="nospelling p" \
			--add-tex-command="prog p" \
			--add-tex-command="author p" \
			--add-tex-command="institute p" \
			--add-tex-command="text p" \
			--add-tex-command="affil  p" \
			--add-tex-command="Refrs p" \
			--dont-tex-check-comments -d en_US -c $$a ;\
		done

spelllist: $(latexfile).rws
		for a in $$(ls -1 $(latexfile)-*.tex); do\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		echo $$a;\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		aspell  --add-extra-dicts=./$(latexfile).rws  -t \
			--add-tex-command="nospelling p" \
			--add-tex-command="prog p" \
			--add-tex-command="author p" \
			--add-tex-command="institute p" \
			--add-tex-command="text p" \
			--add-tex-command="affil  p" \
			--add-tex-command="Refrs p" \
			--dont-tex-check-comments -d en_US list < $$a ;\
		done


clean :
	rm -f $(latexfile)-papers.tex
	rm -f *.aux
	rm -f *.lof
	rm -f *.out
	rm -f *.lot
	rm -f *.bbl
	rm -f *.l4l
	rm -f *.log
	rm -f *.blg
	rm -f *.ilg
	rm -f *.aux
	rm -f $(latexfile)*.dvi
	rm -f $(latexfile)*.ps
	rm -f $(latexfile)*.pdf
	rm -f *.toc
	rm -f *.idx
	rm -f *.ind
	rm -f *.nav
	rm -f *.snm
	rm -f *.rws






